A Hierarchical Pose-Based Approach to Complex Action Understanding Using Dictionaries of Actionlets and Motion Poselets

In this paper, we introduce a new hierarchical model for human action recognition using body joint locations. Our model can categorize complex actions in videos, and perform spatio-temporal annotations of the atomic actions that compose the complex action being performed.That is, for each atomic action, the model generates temporal action annotations by estimating its starting and ending times, as well as, spatial annotations by inferring the human body parts that are involved in executing the action. our model includes three key novel properties: (i) it can be trained with no spatial supervision, as it can automatically discover active body parts from temporal action annotations only; (ii) it jointly learns flexible representations for motion poselets and actionlets that encode the visual variability of body parts and atomic actions; (iii) a mechanism to discard idle or non-informative body parts which increases its robustness to common pose estimation errors. We evaluate the performance of our method using multiple action recognition benchmarks. Our model consistently outperforms baselines and state-of-the-art action recognition methods.

==> composableActivities.tex <==
\subsection{Composable Activities Dataset} \label{subsec:composableActivities}






==> experiments_composable.tex <==
In order to test the suitability of our model for recognition of complex and
composable activities, we use
the Composable Activities benchmark dataset from \cite{Lillo2014}.
This dataset consists of 694 RGB-D
videos that contain activities in 16 classes performed by 14 actors. Each
RGB-D sequence is captured using a Microsoft Kinect sensor, with the
position of relevant body joints estimated using \cite{Microsoft2012}.
Each activity in this dataset is spatio-temporally
composed by a variable number of mid-level (atomic) actions. The total number of
actions in the videos is 25 (plus an \emph{idle} action), while the number of actions
that compose each particular activity fluctuates between 2 to 10 actions.
For instance, the activity \emph{Walking while waving hand} has a spatio-temporal
composition of 2 single actions: \emph{walking} and \emph{waving hand};
while the activity \emph{Composed activity 4} is composed of 10 single actions:
 \emph{walking}, \emph{calling with hands}, \emph{waving hand},
\emph{talking on cellphone}, \emph{picking from floor}, \emph{throwing an object},
\emph{putting an object}, \emph{picking cellphone from pocket}, and \emph{putting
cellphone into pocket}, see Fig. \ref{fig:frontfigure} for some examples.
Every actor performs each activity 3 times in average.
Fig. \ref{fig_activities_actions_table} summarizes the composition of actions for
each activity.
The RGB-D data and annotations for this dataset are publicly available on
our project webpage\footnote{\url{http://web.ing.puc.cl/~ialillo/sparse_hier_activities}}.
%
\begin{figure}[tb]
\begin{center}
\includegraphics[width=0.999\linewidth]{./fig_activities_actions_table.pdf}
\end{center}
\caption{Composition of actions (columns) into activities (rows). Note that some activities are simpler, composed only by two actions, while others are very complex, including up to ten different atomic actions per video. Activities also share an \emph{idle} action, not shown in the table.}
\label{fig_activities_actions_table}
\end{figure}
%

Recognition rates for the Composable Activities Dataset are summarized in Table
\ref{Table-UniNorte}. 
We report performance averaged over multiple runs
using a leave-one-subject-out cross-validation strategy.
We use a validation set to experimentally adjust the value of all the main
parameters.
In practice, we set $\lambda_1 = 100$ and $\lambda_2 = 20$.
We set $K=50$ pose dictionary entries per body region when using the quadratic
regularizer (QR), and $K=150$ per body region when using the sparse
regularizer (SR).
We also reduce the temporal resolution for faster processing by
a factor of 6,
so the effective frame rate for all videos in training and recognition is 5 fps.

\begin{table}
\centering
{\small
\begin{tabular}{|c|c|c|}
\hline
\textbf{Algorithm} & \textbf{GEO} &  \textbf{GEO/MOV}  \\
\hline
Ours, SR+NI& $-$  &  \textbf{92.2\%} \\
Ours, QR+NI& $-$  & 91.8\%  \\
Ours, SR& 84.9\%  & 90.6\%  \\
Ours, QR& 85.7\%  & 90.9\%   \\
\hline
BoW& 67.2\% & 74.1\%    \\
HMM& 76.5\% & 78.9\%  \\
H-BoW& 74.2\% & 82.4\%   \\
2-lev-HIER& 79.6\% & 83.8\%  \\
\hline
LG \cite{vemulapalli2014human} & 74.7\% & $-$  \\
\hline
\end{tabular}
}
\normalsize
\caption{Recognition accuracy of our method compared to several baselines (see text in Section
\ref{subsec:exp_setup}). It is noteworthy that our 3-level model outperforms all 2-levels models. 
Also, as seen in the accuracy for our model, including motion cues in the descriptor (GEO/MOV) and 
using non-informative poses handling (NI) improve the accuracy over our previous model. The best 
performance is obtained when using all the contributions described in this work.
%\JC{JC: Convertir la ultima columna a dos filas: QR + NI, SR + NI}}
}
\label{Table-UniNorte}
%\vspace{-0.4cm}
\end{table}

The confusion matrix obtained with our full model is reported in
Fig.~\ref{fig:confusion_activities}. Note that for some activities the
prediction is perfect, while for others there is high confusion between
some activities, indicating probably highly similar poses like
\emph{calling with hands} and \emph{waving hand}, where many actors
perform the \emph{calling with hands} action with only one arm.

\begin{figure}[tb]
\begin{center}
\includegraphics[width=0.999\linewidth]{./conf_matrix.pdf}
\end{center}
   \caption{Confusion matrix for the activity classification task in the Composable Activities 
dataset, using sparse regularization, a fused descriptor and NI handling.}
\label{fig:confusion_activities}
\end{figure}

To show the semantic interpretation of the poses learned by our model, Fig. 
\ref{fig:example_poses_by_activity} shows top-scoring frames for three activities executed by 
different 
subjects. In general, our model produces highly interpretable poses that are 
associated to characteristic body configurations of the underlying atomic actions. To further 
illustrate this observation, Fig. \ref{fig:poses} shows the highest activations for eight pose 
dictionary entries associated to the body region corresponding to the left arm. In each case, 
Fig. \ref{fig:poses} also indicates the atomic action that assigns a greatest relevance (weight) to 
the corresponding pose. 
%\JC{Alvaro: No entiendo bien la ultima frase. Ademas, uno de los revisores pidio mostrar figuras de las poses aprendidas por el metodo. Podemos unir con esto?. Quizas mostrando con algun color el area de la pose identificada. O ejemplos caracteristicos de las poses, como en el paper de Bourdev and Malik sobre poselets (ECCV, 2012).}

\begin{figure}[tb]
\begin{center}
\includegraphics[width=0.999\linewidth]{./fig_examples_poses_by_activity.pdf}
\end{center}
   \caption{Examples of top score frames for three activities. Note the high correlation between the actions that compose each activity and the pose of the actors.}
\label{fig:example_poses_by_activity}
\end{figure}


\begin{figure}[tb]
\begin{center}
\includegraphics[width=0.999\linewidth]{./fig_poses.pdf}
\end{center}
   \caption{Examples of top scored poses for the body 
region corresponding to the left arm. Also shown, it is the label of the action with 
the highest classifier weight associated to the pose. In this case the model is trained using SR 
and $K=150$ for 
each body region.}
\label{fig:poses}
\end{figure}

As shown in Table \ref{Table-UniNorte}, we place our recognition results in context by comparing 
them to the performance of
two baselines methods, two simplified versions of our model, and a state-of-the-art algorithm.
The first baseline is based on a bag of words framework
(BoW), which only captures very coarse per-region
pose orderings and uses an independently pre-trained pose dictionary. Specifically, 
this baseline uses $k$-means to quantize pose descriptors
for each body region independently, which are aggregated into
a temporal pyramid histogram representation.
This is then fed into a multi-class linear SVM
for directly mapping from video descriptors to activities. 
The accuracy of this
baseline is 74.1\% when using the combined
descriptor based on geometric and motion information.

As a second baseline, we implement a Hidden Markov Model (HMM).
The HMM model can directly encode pose and action transitions built
upon an independently pre-trained pose dictionary.
In our implementation, states are trained with supervision by assigning one
state to each atomic action. Quantized poses are the observed variables.
We train models independently for each class, and at testing time,
we classify new sequences by assigning the label that corresponds to the
highest scoring model. The accuracy of this
baseline is 78.9\% when using the combined
descriptor based on geometric and motion information. While the ordering encoded by the HMM model 
helps to improve accuracy over BoW,
it still lacks the discriminative power of the top layer in our model for
jointly learning model parameters for all classes. 


We also compare performance against two simplified versions of our hierarchical
model. The first simplified version (H-BoW) does not jointly
learn the pose dictionary, but uses a fixed pose quantization obtained with
$k$-means, and omits the transition terms.
Unlike our full model, this simplified version does not take advantage of
jointly learning the pose dictionary, which leads to sub-optimal
pose encoding at the lower level of the hierarchy.
Also, by omitting the transition terms, the model cannot capture patterns
in the evolution of actions and poses.
These simplifications lead to a 10\% drop in performance in comparison
to our full model.

As a second simplification of our full model, we construct a
hierarchical model (2-lev-HIER) with two jointly learned
layers that encode poses and atomic actions. Activity recognition
is performed by an independently trained linear
classifier on top of the inferred atomic actions.
In this case, the performance of this model simplification is 8.4\% lower
than our full model. It is interesting that even when seemingly the top two
levels are uncoupled and one could train them independently,
there are benefits in jointly learning them.
%The action prediction in our 3-level hierarchical model is highly
%connected to the activity that is imputed during classification
%(recall that for classification we exhaustively search for each activity which
%produces the highest scored sequence of actions and poses, as
%Equation (\ref{eq:classify_inference})).
%Finally, jointly learning the pose dictionary is also beneficial, 
%as we gain about 3\% in accuracy when compared to
%using a pre-trained pose dictionary.


We also compare against an existing state-of-the-art algorithm from
the literature. In this case, we compare to the
method recently described in \cite{vemulapalli2014human} (LG).
%Another simple model is LG \cite{vemulapalli2014human},
We select this algorithm because it achieves state-of-art
performance on several pose-based action datasets. We train this model to
directly predict the activities from poses, omitting the mid-level
annotations, as in the BoW baseline. While the accuracy of LG is above BoW, it is
still 11\% lower than our model that only uses geometric information (GEO).

%\JC{General comments}:
%
%It is worth to note that all baselines that omit the mid-level
%(atomic actions) annotations (BoW and LG) perform worse that the the others
%that use that information.
%
%Our results confirm that jointly learning the
%classifiers in three levels (activities, actions and poses) outperform simpler
%setups by around 10\% of accuracy.


==> experiments_detailed_CA.tex <==
%We use $K = 50$ poses for each body part (a total of 200 poses), 
%which provides a good compromise between computational load and recognition accuracy.
%Our method is relatively robust to the size of the pose dictionary. A low
%number of poses per body part (5 to 20) lacks representativity, and a
%high number increases the computational load and increases over-fitting. In our
%experiments, we observe similar performance for the case of 50, 100 and 150
%poses per body part. When testing with 25 poses the accuracy drops by 6\%. We did not test larger
%dictionaries due to high processing time, which is quadratic with respect to
%dictionary size.

\subsection{Inference of per-frame annotations.}
\label{subsec:action_annotation}
The hierarchical structure and compositional
properties of our model enable it to output a predicted global activity,
as well as per-frame annotations of predicted atomic actions and poses for each body
region.
It is important to highlight that in the generation of the per-frame annotations, no prior temporal 
segmentation of atomic actions is needed. Also, no post-processing of the output is performed. The  
proficiency of our model to produce
per-frame annotated data, enabling action detection temporally and
spatially, make our model unique. 

Figure \ref{fig:annotation} illustrates
the capability of our model to provide per-frame annotation of the atomic
actions that compose each activity. The accuracy of
the mid-level action prediction can be evaluated as in \cite{Wei2013}.
Specifically, we first obtain segments of the same predicted action in each
sequence, and then compare these segments with ground truth action labels. The
estimated label of the segment is assumed correct if the detected segment is
completely contained in a ground truth segment with the same label, or if the
Jaccard Index considering the segment and the ground truth label is greater
than 0.6. Using these criteria, the accuracy of the mid-level actions is
79.4\%. In many cases, the wrong action prediction is only highly local in time
or space, and the model is still able to correctly predict the activity label
of the sequence. Taking only the correctly predicted videos in terms of global
activity prediction, the accuracy of action labeling reaches 83.3\%. When consider this number, it 
is
important to note that not every ground truth action label is accurate: the
videos were hand-labeled by volunteers, so there is a chance for mistakes in
terms of the exact temporal boundaries of the action. In
this sense, in our experiments we observe cases where the predicted
labels showed more accuracte temporal boundaries than the ground 
truth.
%As an example, in
%some videos a walking action that last only a few frames is correctly
%predicted, where it was not identified during the labeling process, but it lead
%to errors in the action prediction.
%\JC{Alvaro: aclarar ultima frase}

 
\begin{figure*}[th]
\begin{center}
\includegraphics[width=0.999\linewidth]{./fig_all_sequences_red.pdf}
%\includegraphics[width=0.999\linewidth]{./fig_examples_action_annotation.pdf}\\
%\includegraphics[width=0.999\linewidth, trim= 0 0 200 0, clip]
%{./subject_1_32.pdf}\\
%\includegraphics[width=0.999\linewidth]
%{./subject_2_21.pdf}\\
%%\includegraphics[width=0.95\linewidth]
%%{./subject_6_23.pdf}\\
%\includegraphics[width=0.999\linewidth]
%{./subject_6_30.pdf}\\
%%\vspace{-0.5cm}
\end{center}
\caption{Per-frame predictions of atomic actions for selected activities,
showing 20 frames of each video. Each frame is joined with the predicted action
annotations of left arm, right arm, left leg and right leg. Besides the prediction of the global 
activity of the video, our algorithm is able to
correctly predict the atomic actions that compose each activity in each frame,
as well as the body regions that are active during the execution of the action.
Note that in the example video of the activity \emph{Walking while calling with
hands}, the \emph{calling with hands} action is correctly annotated even when
the subject change the waving hand during the execution of the activity.}
%\vspace{-0.4cm}
\label{fig:annotation}
\end{figure*}

\subsection{Robustness to occlusion and noisy joints.}
Our method is also capable of inferring action and activity labels even if some
joints are not observed. This is a common situation in practice,
as body motions induce temporal self-occlusions of body regions.
Nevertheless, due to the joint estimation of poses, actions, and activities,
our model is able to reduce the effect of this problem. To illustrate this, we
simulate a totally occluded region by fixing its geometry to the position
observed in the first frame.
We select which region to be completely occluded in every sequence using uniform sampling.
In this scenario, the accuracy of our preliminary model in \cite{Lillo2014} drops
by 7.2\%. Using our new SR setup including NI handling, the accuracy only drops
by 4.3\%, showing that the detection of non-informative poses helps the model
to deal with occluded regions. In fact, as we show in Section
\ref{subsec:exp_non_info_handling}, many of truly occluded regions in the
videos are identified using NI handling. In contrast, the drop in performance of
BoW is 12.5\% and HMM 10.3\%: simpler models are less capable of robustly dealing
with occluded regions, since their pose assignments rely only on the descriptor
itself, while in our model the assigned pose depends on the descriptor,
sequences of poses and actions, and the activity evaluated, making inference
more robust. Fig. \ref{fig:occlusions} shows some qualitative results of
occluded regions.

%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=0.95\linewidth]{./jc/M_actionG_C2000_SUB.pdf}
%\includegraphics[width=0.95\linewidth]{./jc/M_actionG_optim.eps}
%\vspace{-0.5cm}
%\end{center}
 %  \caption{Confusion matrix for the action classification task. Rows are the
%ground truth actions at each frame, while columns are the predicted
%mid-level action label inferred by our model.}
%\label{fig:confusion_actions}
%\vspace{-0.4cm}
%\end{figure}

\begin{figure}[tb]
\begin{center}
%\fbox{\rule{0pt}{0.5in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=0.999\linewidth]
{./subject_1_6.pdf} \\
{\footnotesize Right arm occluded} \\
%\fbox{\rule{0pt}{0.5in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=0.999\linewidth]
{./subject_1_23.pdf}\\
{\footnotesize Left leg occluded}  \\
%\fbox{\rule{0pt}{0.5in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=0.999\linewidth]
{./subject_1_8.pdf}\\
{\footnotesize Left arm occluded}\\
%\vspace{-0.3cm}
\end{center}
\caption{The occluded body regions are depicted in light blue. When an arm or
leg is occluded, our method still provides a good estimation of the underlying actions in each
frame.}
\label{fig:occlusions}
%\vspace{-0.6cm}
\end{figure}

In terms of noisy joints, we manually add random Gaussian noise to change the
joints 3D location of testing videos, using the SR setup and the GEO descriptor
to isolate the effect of the joints and not mixing the motion descriptor. Figure
\ref{fig:joint_noise} shows the accuracy of testing videos in terms of noise
dispersion $\sigma_{noise}$ measured in inches. For little noise, there is no
much effect in our model accuracy, as expected for the robustness of the
geometric descriptor. However, for more drastic noise added to every joint, the
accuracy drops dramatically. This behavior is expected, since for highly noisy
joints the model can no longer predict well the sequence of actions and poses.   

\begin{figure}[tb]
\begin{center}
%\fbox{\rule{0pt}{1in} \rule{0.999\linewidth}{0pt}}
\includegraphics[width=0.999\linewidth]{./fig_acc_vs_noise.pdf} \\
\end{center}
\caption{Performance of our model in presence of simulated Gaussian noise in
every joint, as a function of $\sigma_{noise}$ measured in inches. When the
noise is less than 3 inches in average, the model performance is not very
affected, while for bigger noise dispersion the model accuracy is drastically
affected. It is important no note that in our simulation, every joint is
affected to noise, while in a real setup, noisy joint estimation tend to occur
more rarely. } \label{fig:joint_noise}
\end{figure}

\subsection{Early activity prediction.}
Our model needs the complete video to make an accurate activity and action
prediction of a query video. In this section, we analyze the number of frames
(as a percentage of a complete activity sequence) needed
to make an accurate activity prediction. Figure \ref{fig:accuracy_reduced_frames}
shows the mean accuracy over the dataset (using leave-one-subject-out
cross-validation) in function of the
percentage of frames used by the classifier to label each video. We note that
considering 30\% of the frames, the classifier performs reasonable predictions,
while 70\% of frames are needed to closely match the
accuracy of using all frames.
\begin{figure}[tb]
\begin{center}
\includegraphics[width=0.999\linewidth]{./fig_acc_vs_frame_reduction.pdf}
\end{center}
\caption{Accuracy of activity recognition versus percentage of frames used in
Composable Activities dataset. In general, 30\% of the frames are needed to
perform reasonable predictions, while 70\% of frames are needed to closely match the
accuracy of using all frames.}
\label{fig:accuracy_reduced_frames}
\end{figure}

\subsection{Failure cases.}

We also study some of the failure cases that we observe during the
experimentation with our model.
%As all models, there will be a few errors in the predicted activity for testing
%videos.
Figure \ref{fig:errors} shows some error cases. It is interesting that
the sequences are confusing even for humans when only the skeleton is available
as in the figure. These errors probably will not be surpassed with the model
itself, and will need to use other sources of information like object
detectors, where a cup should be distinguished from a cellphone as in the
third row of Figure \ref{fig:errors}.

\begin{figure}[tb]
\begin{center}
%\fbox{\rule{0pt}{0.5in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=0.999\linewidth]
{./sbj1_1.pdf} \\
{\footnotesize Ground truth: Walking while calling with hands\\
Prediction: Walking while waving hand} \\
%\fbox{\rule{0pt}{0.5in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=0.999\linewidth]
{./sbj4_4.pdf}\\
{\footnotesize Ground truth: Composed activity 1\\
Prediction: Talking on cellphone and drinking}  \\
%\fbox{\rule{0pt}{0.5in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=0.999\linewidth]
{./sbj4_6.pdf}\\
{\footnotesize Ground truth: Waving hand and drinking\\
Prediction: Talking on cellphone and scratching head} \\
%\vspace{-0.3cm}
\end{center}
\caption{Failure cases. Our algorithm tends to confuse activities that share very similar
body postures.}
%\JC{Alvaro: podria mejorarse, pero no es algo importante}}
\label{fig:errors}
%\vspace{-0.5cm}
\end{figure}


\begin{comment}
\subsubsection{New activity characterization}
As we mention in previous section, our model using sparse regularization and
non-negative weights on activity ($\alpha$) classifiers and action ($\beta$)
classifiers do not \emph{punish} poses that have no influence in the
activities. For this reason, our model is able to model a new composed activity
just combining the coefficients of two known activities, leaving the rest of
the parameters of the model untouched. We use an heuristic approach to combine
two models: givint two classes $c_1$ and $c_2$, their coefficients for a region
$r$ and action $a$ are $ \alpha^r_{c_1,a}$ and $ \alpha^r_{c_2,a}$
respectively. For a new class $c_{new}$ composed of classes $c_1$ and $c_2$, we
use the mean value of the coefficients \begin{equation}
\alpha^r_{{c_{new},a}} = \frac{(\alpha^r_{c_1,a} + \alpha^r_{c_2,a})}{2}
\end{equation}
 only when the corresponding coefficients for are positive; in other case, we
use the maximum value of the two coefficients. For all subjects of the dataset,
we create all the combinations od two activities, and tested the new model
using three composed videos per subject. The average accuracy of the activity
$16+1$ is 90.2\%, and in average the activities that compose the new activity
drops its accuracy in 12.3\%, showing that we effectively incorporate a new
composed activity to the model at a little cost of getting more confusion over
the original activities. Moreover, the accuracy of action labeling for the new
class is 74.2\%,  similar to the accuracy of the action labeling of the
original model, so we can effectively transfer the learning of atomic action
classifiers to new compositions of activities. 

\begin{table}
\begin{tabular}
\hline
Activity group & Accuracy of new class & \\ 
\hline
Simple & 92.2% &  \\
Complex & 87.2\% & \\
\hline
All & 90.2\% & \\
\end{tabular}
\caption{}
\label{tab:acc_new_class}
\end{table}

\end{comment}


==> experiments_motion.tex <==
In the preliminary version of our model \cite{Lillo2014},
we describe each frame using cues related to the geometry of the skeleton joints (GEO).
%we only use body joint positions from the estimated skeleton to compute our descriptor,
%disregarding valuable RGB motion information.
In this paper, we augment the representation by including a dynamic descriptor
that captures local dynamic information
as described in Section \ref{subsec:videorepresentation}. As reported in Tables \ref{tab:msr} and 
\ref{Table-UniNorte}, we present experimental results using the geometric descriptor (GEO), as well 
as the fused descriptor (GEO/MOV).

It is important to note that giving that the MSR-Action3D dataset does not include RGB information,
we modify the motion descriptor described in Section 
\ref{subsec:videorepresentation}. Specifically,
we encode differences of displacements for every joint, in a similar setup to
\cite{WangCVPR2011}.
This results in an 18 dimensional motion descriptor for each body region,
since each region contains 6 joints and each joint is a 3D vector.
The preliminary the version of our model \cite{Lillo2014} that uses
a quadratic regularizer and geometric features only,
we achieve a classification accuracy of 89.5\%.
By incorporating dynamic features,
we achieve an action classification accuracy of 90.6\%, reducing the error by 1.1\%. In the 
Composable Activities dataset, we use the motion descriptor described in Section 
\ref{subsec:videorepresentation}.
By adding the dynamic descriptor, the
improvement in accuracy is more notorious than in MSR-Action3D,
reducing the error by 5.2\% and 5.7\% according to the use of QR or SR regularizers, respectively.

Fig. \ref{fig:geo_mov_importance} shows the relative weight
of the geometric descriptor and motion descriptor in relation to each activity class
for the right arm and right leg. Focusing on right arm (left graph), note that
for actions like \emph{scratching head}, \emph{throwing an object} or
\emph{erasing the board}, the geometry of the joints is relatively more
important that the motion cues. Inversely, for other actions like
\emph{gesticulating} or \emph{calling with hands} the motion descriptor is more
important in average, since for these actions the movement of the arm is where
the information is encoded. 

\begin{figure}[tb]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.999\linewidth}{0pt}}
\includegraphics[height=2.2 in]{./fig_desc_relative_right_arm_mod.pdf}
\includegraphics[height=2.2 in]{./fig_desc_relative_right_leg_mod.pdf}
\end{center}
\caption{Relative importance of geometric (GEO) and motion (MOV) descriptors for right arm (left) and right leg (right).}
\label{fig:geo_mov_importance}
\end{figure}


==> experiments_non_info_handling.tex <==
In our framework, we include a mechanism to identify and discard non-informative poses (NI) 
appearing in some frames. The mechanism assigns a learnable score $\theta$ to frame poses
that are non-informative to the action classifier
(see Eq. (\ref{Eq_poseEnergy})).
The poses from these frames are not accumulated into the pose histograms that
are fed to the action classifiers.
This enables to model to focus on more discriminative poses, which results in
more discriminative classifiers.

During learning, we need to initialize the set of candidate frame poses that can be considered 
as NI.
In practice, we initialize the NI poses by using the initial pose
dictionary obtained with $k$-means, and selecting as NI the poses that are
most distant to their assigned cluster centers. For each video,
we initially assign a total of 20\% of the frames to the NI bucket.
%To initialize training, during the first step of the learning algorithm the NI
%frames are assigned to be the 20\% of the most disperse frames, in terms of the
%distance to the assigned cluster center computed with $k$-means.
As the learning progresses, on each iteration poses can be reassigned to
a pose dictionary entry or to NI. In general, we observe that after convergence approximately 
17\% of all training frames are assigned as non-informative.
When we initialize the NI assignment with 40\% of the frames,
our final model reduces this to 19\%.
This indicates that
our model is effectively learning to detect non-informative frames in
the training videos.
%A similar behavior is observed when selecting 40\% of frames as initial
%non-informative frames, ending with 19\% of non-informative frames. This shows
%the dataset, and opens an entire field to test the same idea in, for example,
%patch-based object recognition.
%On the other hand,
%Also, 65\% of the initial NI poses were reassigned to a pose dictionary entry,
Moreover, near 40\% of the initial pose assignments are updated throughout
the iterations. This is compared to 25\% in preliminary model without
non-informative pose handling. This indicates that our full model is capable of
updating the pose representations more effectively.

In terms of accuracy, the use of NI reduces the error in 1.8\% in
MSR-Action3D, raising the accuracy from 90.6\% to 92.4\%. In the Composable Activities dataset the 
introduction of NI causes the error to
drop 1.4\% when using the SR regularizer, for a recognition accuracy of 92.2\%.
%

An important ability of the NI mechanism is that occluded regions are often
assigned as NI poses. Figure \ref{fig:non_info_poses_sequence} shows a
sequence of the activity \emph{Walking while reading}. In this figure, the bottom graph shows with 
black boxes frames where a body region is identified by our method as corresponding to a 
non-informative pose. Observing the body region corresponding to the arms, the long sequences of 
non-informative
poses nearly coincides with the occlusion periods of the arms (thick gray lines). Other frames
considered as non-informative tend to be sparser in time, and they can be
explained by rare poses or noisy body joints estimation. This behavior is
advantageous in two ways: during learning, it allows the model to
automatically disregard many occluded regions when learning the pose
classifiers; and during testing, it allows the model to identify possible occluded regions.

\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.999\linewidth]{./fig_non_iinfo_poses.pdf}
\end{center}
\caption{\textforreview{Non-informative pose sequence for the four regions of
the body, in a video from the activity \emph{Walking while reading}. The black
squares represent frames labeled as a non-informative pose. A thick gray line
shows when the corresponding region is occluded. We can observe a relation between body region 
occlusions and identification of non-informative poses. Specifically,  when there is no occlusion, 
the identification of non-informative poses
tends to be temporally sparse, but for occluded intervals, many consecutive
frames are selected as non-informative.} } \label{fig:non_info_poses_sequence}
\end{figure*}

Figure \ref{fig:NI_handling} shows a comparison of some learned pose dictionary
entries with and without NI handling related to the activity \emph{Composed
Activity 5}, whose main atomic actions are \emph{walking},
\emph{gesticulating}, \emph{erasing board} and \emph{writing on board}. We show
the best-scored and worst-scored frames where two or more body regions are not
\emph{idle} or labeled as non-informative, i.e., correspond to poses that are
supposed to be discriminative for the activity.
Figure \ref{fig:NI_handling} illustrates that when using NI handling, the worst scored
frames imputed
as informative still preserve the semantics of the actions performed, while
without NI, the worst poses are noisy and without real meaning for the
performed action. Moreover, the non-informative frames in the right
clearly show poses that are not specific to the activity (or any activity),
and are correctly labeled as non-informative poses. This shows that using NI handling also helps 
to increase the semantic interpretation of the learned pose classifiers.

\begin{figure*}[tb]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.999\linewidth}{0pt}}
\includegraphics[width=0.999\linewidth]{./fig_NI_poses.pdf}
\end{center}
\caption{Comparison of frames showing poses from videos of the activity
\emph{Composed Activity 5}. All the presented frames belong to a subset of
frames where there is at least two body regions active for the underlying action
(not \emph{idle}). The best-scored
frames are similar with both setups. However, when considering the worse-scored
frames, it is clear that for the original model there are poses that are
not helping to the activity prediction. In general, those poses are labeled as
non-informative with our proposed modification, where the worse-scored poses of the new model
still remain discriminative and semantically valid for the target activity.}
\label{fig:NI_handling}
\end{figure*}


==> experiments_simple.tex <==
%We report results on two publicly available datasets:
%the MSR-Action3D \cite{WanLi2010} dataset for benchmarking recognition of simple actions,
%and our Composable Activities Dataset introduced in \cite{Lillo2014}.
%We next describe each dataset as well as some implementation details.

While our model is aimed at the recognition of activities that can be composed by simpler actions,
we experimentally verify that the model can also handle the case of simple action recognition.
Towards this goal, we evaluate our algorithm on the MSR-Action3D dataset \cite{WanLi2010},
which consists of 10 subjects performing 20 actions related to gaming in front of a TV.
This dataset provides skeleton data (joint locations) and low resolution depth maps.

During training, our hierarchical model needs 
a global activity label as well as per-frame atomic action labels. However, the MSR-Action3D 
dataset only includes the annotation of a single global action for each video. As a consequence, 
we need to augment the annotations of this dataset to be compatible with our model. To achieve 
this, we automatically augment the annotations as follows. At the activity level of our model, we 
use the original action label provided in the dataset as our global activity
label. Similarly, at the atomic action level of our model, 
we annotate each video frame with this global action label. As a further adaptation, we swap to an
\emph{idle} label all inactive frames. We select the frames annotated as \emph{idle} following a 
simple heuristic. First, we annotate as 
\emph{idle} the four body regions of the first frame of each video. Then, we search for all frames 
in which the pose of each region closely resembles the corresponding pose in
the first frame, labeling all these regions as \emph{idle} too. This simple heuristic works well to 
identify \emph{idle}
frames in this dataset, since subjects start the video
with a resting position. Additionally, we filter out noisy \emph{idle} labels by 
only keeping as such sets of more than 6 consecutives frames labeled as \emph{idle}. Finally, 
we assign a complete region in a video as \emph{idle} if this label appears in more than 60\% of 
the 
frames.

In our experiments, we use a total of 552 sequences.
We omit 5 out of the 557 videos because they have missing joints in
the last half of the sequence.
We test our model on all 20 action categories using cross-subject validation,
with subjects 1-3-5-7-9 for training and the rest for testing.
This corresponds to the same experimental setting used in \cite{Wang2012}.
In our evaluation, we use $K=100$ poses for each body region, for a total of 400 pose 
dictionary entries.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
%{\small
\begin{tabular}{|c|c|}
\hline
\textbf{Algorithm} & \textbf{Accuracy}\\
\hline
Ours  &  \textbf{92.4\%} \\
\hline
%J. Luo et al. \cite{luo2013group} & \textbf{96.7\%} \\
%Y. Zhu et al. \cite{zhu2013fusing} & 94.3\% \\
C. Wang et al.\cite{Wang2013} &    90.2\% \\
Vemulapalli et al. \cite{vemulapalli2014human} & 89.5\% \\
Lillo et al. \cite{Lillo2014} & 89.5\%\\
Xia and Aggarwal \cite{Xia} & 89.3\% \\
J. Wang et al. \cite{Wang2012} &   88.2\% \\

\hline
\end{tabular}
%}
\caption{Recognition accuracy of our approach in the MSR-Action3D dataset compared to other
methods in the literature that also use the experimental setup in 
\cite{Wang2012}. Our method improves state-of-the-art
performance in this dataset.
%We include methods that use
%joint data only and evaluation using cross-subject using all 20 action categories.
}
%\vspace{-0.3cm}
\label{tab:msr_st}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
Table \ref{tab:msr_st} reports the overall recognition accuracy of our model
in the MSR-Action3D dataset,
as measured by the average of the diagonal of the normalized confusion matrix. Additionally,
Table \ref{tab:msr_st} compares our results to alternative methods proposed in the literature
that also use the training/testing setup proposed in \cite{Wang2012}.
Under this experimental setting, our model improves the state-of-art accuracy
in this dataset.

%\JC{Alvaro: queda cojo pues finalmente solo se reporta el accuracy como todos
%los otros modelos. Hay que conectar esto con algun resultado cuantitativo o
%cualitativo que muestre las ventajas indicadas}
In addition to the strong activity recognition performance, our model
has also the advantage of generating a rich video interpretation in the form of
detailed per-frame and per-body-region action annotations.
In contrast, all competitive models only produce a coarse interpretation
in the form of a global video label prediction. Section \ref{subsec:action_annotation} provides 
quantitative and qualitative insights about the capabilities of our method to infer at each frame 
the body regions executing the action.

An important aspect of these results is that our model achieves
this performance using a pose dictionary of only 100 entries per region.
This compares favorably with the results reported in \cite{Wang2012}, \cite{Wang2013}, and 
\cite{Xia},
which use dictionaries with thousands of entries.
Our reduced dictionary translates to more compact models that require
less computation at the inference stage. 

%Furthermore, our model does not require a previous 
%temporal segmentation as \cite{Koppula2012} or \cite{Wei2013}, the 
%inputs to our model are only the frame descriptors.

%As we will see in Section \ref{subsec:sparse_reg}, using a larger pose dictionary does not produce 
%necessarily better results in our model, as well as a huge increasing in $K$ will make the 
%inference impractical since the computing time is proportional to $K^2$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\begin{table}
\centering
%{\small
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Algorithm} & \textbf{GEO} & \textbf{GEO/MOV} & \textbf{GEO/MOV + NI} \\
\hline
Ours, QR  &  89.5\% & 90.6\% & \textbf{92.4\%} \\
\hline
\end{tabular}
%}
\caption{Recognition accuracy of our approach in MSR-Action3D using a quadratic regularizer 
(QR) and different settings: i) Using only a geometric 
descriptor (GEO), ii) Combining  a geometric and a motion descriptors (GEO/MOV), and iii) Adding a 
mechanism to identify and discard non-informative poses (NI).}
%\vspace{-0.3cm}
\label{tab:msr}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\JC{Alvaro: mover a mas adelante, donde se explican los efectos indicados,
%i.e., secciones 4.3 y 4.4.}
Finally, Table \ref{tab:msr} reports the performance of our model
under several settings. First, we report performance when
the model uses a quadratic regularizer (QR)
combined with the geometric descriptor described in Section 
\ref{subsec:videorepresentation} (GEO). This corresponds to the setup used in 
\cite{Lillo2014}. We also consider the case when we combine the geometric descriptor with the 
motion 
descriptor described in Section 
\ref{subsec:videorepresentation} (GEO/MOV). Additionally, we consider the case when the model 
includes the 
proposed method to identify and discard non-informative (NI).
We further discuss the effect of these settings in the following sections.

%We report the overall recognition accuracy as measured by the average of the
%diagonal of the normalized confusion matrix.
%We specify in the experiments when the 
%quadratic regularizer (\textbf{QR})
%or sparse regularizer (\textbf{SR}) is applied, as well as if the descriptor
%used is only geometric (\textbf{GEO}), or a fused descriptor including geometry
%and motion (\textbf{GEO/MOV}). We also specify when the handling of
%non-informative poses is applied (\textbf{NI}).


==> experiments_sparse_reg.tex <==
%\JC{Alvaro: El primer parrafo repite la explicacion ya presentada en seccion 3.4.}
%In this paper, we have extended our model by introducing sparse
%regularization to improve the use of poses in the dictionary.
%In the preliminary version of our framework \cite{Lillo2014}, the model
%parameters are optimized using a quadratic regularization, leading to unregularized pose assignments.
In this paper we extend our preliminary model by introducing
a new regularizer that consists of a mixture of $L_2$ and $L_1$
norms for the atomic action
classifiers $\beta$ (see Equation \ref{eq:general_regularizer}).
The goal of the new regularization is to obtain a more
efficient use of the dictionary of body poses, in the sense that the model
learns more specialized poses for each atomic action, which also encourages
the fewer poses to be influential for each activity. For testing the effects of
sparse regularization in $\beta$, we use the Composable Activities dataset since
it provides richer hierarchical annotations.
We use fixed values $\mu=0.1$ and $\rho=5$ of
Eq. (\ref{eq:general_regularizer}) using sparse regularizer
(SR), contrasting the usual values used for $L_2$ regularizer (QR) $\mu=1$ and
$\rho=0$. Also, for QR setup, the number of poses is set to $K=50$ per body
region, while for SR is set to $K=150$ per body region.

In our experiments, we observe that when using SR only 8 to 11\% of the coefficients of $\beta$
remain non-zero. In average, this means a reduction of 85\% in the number of non-zero terms 
with respect to the use of QR. In terms of accuracy, as we see in Table \ref{Table-UniNorte},
recognition performance using sparse regularizer (SR) is similar to the case of
a quadratic
regularizer (QR), decreasing the error in 0.4\% when using the fused descriptor
and NI handling, and slightly increasing the error when the other modifications
are not applied. Despite the similar recognition accuracy provided by both regularizers, we 
identify at least three relevant advantages of using the SR setup:

\paragraph{i) Increased robustness to overfitting problems when using a sparse regularizer.} Figure 
\ref{fig:acc_vs_K_CA} shows recognition accuracy in function of the pose dictionary size $K$ when 
using QR and SR in
the Composable Activities dataset. We observe that when using QR the model clearly overfits as the 
dictionary grows larger than $K=50$. In contrast, using the SR setup, the
accuracy tends to increase or at least hold when larger dictionaries are used.
This behavior shows that the model using SR regularizer is best suited to be used
in larger models, since the learned poses are more specialized, and the model shows an 
increased robustness to overfitting problems. 

\begin{figure}[tb]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.999\linewidth}{0pt}}
\includegraphics[width=0.999\linewidth]{./fig_acc_vs_K.pdf}
\end{center}
\caption{Accuracy of testing versus the number of pose dictionary entries per
body region ($K$), for QR and SR setups. Note the decreasing accuracy of QR
setup (quadratic regularizer), indicating overfitting when more pose dictionary
elements are used, whereas using a sparse regularizer (SR) the accuracy remains
almost with no change. } \label{fig:acc_vs_K_CA}
\end{figure}

\paragraph{ii) Fewer poses influence each activity.}
One of the goals of using a sparse regularizer is to decrease the number of
entries from the pose dictionary that are used by each action classifier.
Since few pose dictionary entries
are required to explain each action (and therefore each activity),
this encourages every action to rely on a smaller group of poses, which usually
helps in improving the generalization power of the model,
the semantic interpretability of the poses,
and the efficiency of the pose dictionary.
%The
%influence (Eq. (\ref{XX})) of the poses aggregated for all activities
%and \ref{fig:poses_decay_C6}. Note the fast decay for pose influence when
%using the
%sparse regularizer, meaning that the model will focus on less poses when inferring the
%activity and actions of the video. Also, note the less decay in a more complex
%activity like \emph{Composed Activity 6} compared to \emph{Walking while hand waving};
%more poses influence the classification when the activity is more complex.
To illustrate this behavior, Figure \ref{fig:influence_agg} includes two diagrams corresponding to 
the influence (measured by Eq. (\ref{eq:influence})) of the
pose dictionary entries of right arm, across all activities, for QR setup (top
diagram) and SR setup (bottom diagram). We binarize the influence using a threshold
corresponding to the 5\% of the top influence value, to better showcase the
grouping effect.  For a fair comparison, $K=50$ is used in both setups, and we
use the same initial pose labels $Z$ to make the poses comparable. It is clear
from the figure that in the QR setup each activity is influenced by many poses
(and therefore each pose entry has activations in many activities), without a
clear pattern of pose activations. In this setup, 17.8 pose entries
influence each activity in average;
in contrast, for SR setup, only 8.6 poses in
average are influential for each activity, showing a sparse pattern. Since the
pose dictionary and atomic action classifiers are shared by all activities, the
grouping effect is straightforward, since the activities that share a common
action will also share its poses. As an example, if we observe the activations for the 
three activities
composed by the action \emph{Talking on cellphone}, many common poses are shared by these three
activities, and few of them are not, showing a grouping effect. Moreover, for those activities that 
do not
share atomic actions, the poses tend to be also non-shared. We omit from the
analysis the \emph{idle} action to enforce the influence of actual annotated
actions.

\begin{figure}[tb]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.999\linewidth}{0pt}}
\includegraphics[width=0.999\linewidth]{./fig_influence_QR_vs_SR.pdf}
\end{center}
\caption{Graphical representation of the influence of right-arm poses (using
$K=50$) in the activities of the Composable Activities dataset, using quadratic
regularizer (QR) and sparse regularizer (SR) (black is for influence score above a given 
threshold). Note that the SR setup
allows each activity to be represented by fewer poses, increasing the
interpretability of the poses generated by the model and the efficiency in pose
usage.
%\JC{JC: Aqui negro es desactivo, en la fig 9, negro indica activo. Es un poco confuso...}
%\JC{Alvaro: Seria posible generar una figura en que se cambia el orden del eje
%X. Tal que se ordena segun hamming distance (in a binary vector como cada
%columna de la figura), esto deberia permitir la visualizacion de grupos.
%Tambien se podria reportar el numero promedio de features usadas en figuras a
%y b para mostrar la reduccion del numero de poses usadas por cada clase.}
}
\label{fig:influence_agg}
\end{figure}
%
\paragraph{iii) Improved semantical interpretation of poses.}
The SR setup helps to improve the semantic meaning of the learned poses.
Observing Fig. \ref{fig:influence_agg}, the learned poses are
related to the actions involved in the activities. For example, just considering
poses 1 to 5 in the figure, we observe that in the SR setup they influence
the activities \emph{Composed Activity 4}, \emph{Waving hand and drinking}, and
\emph{Walking while waving hand}. It is clear that this 
group of poses correspond to the
right arm body region. Furthermore, they are related to the \emph{waiving hand} action, since 
it is the only
action that appears in all these activities. This kind of interpretation is not
possible under the QR setup. We foresee that the relevance of this type of interpretations can 
increase as new recognition scenarios will require the interpretation
of a larger number of actions. Note that we omit the \emph{idle} action when computing the influence scores for clarity (all activities share the\emph{idle} action), that is why some rows of Fig. \ref{fig:influence_agg} are all white (not influential to any activity).

%Additionally, we force the
%coefficients of the activity and atomic action classifiers to be positive, forcing the
%model to focus in the poses actually \emph{present} in each action and activity, and
%not \emph{punishing} the poses that should not be present. It is remarkable that using
%only positives weights for $\alpha$ and $\beta$, and also using small groups of poses
%for each $\beta$, the recognition accuracy is the same as the more unconstrained
%discriminative problem. We see several advantages in using the sparse regularizer with
%positive weights: the model does a more efficient use of the pose dictionary, as higher level
%classifiers only see relevant poses. By using only positives weights in the higher level
%classifiers, we are fostering the model to behave similarly to a generative model, so
%merging two activities to create a new composed activity could be made at no cost.
%%; we
%%will explore this property as part of our future work.
%Also, the positive weights
%force the model to focus on present actions in the videos, making the activity
%classifiers naturally sparse.



%\textforreview{
%In addition to the regulaizer, the extended model also adds a new term into
%the loss function that
%penalizes the diversity of learned poses inside an executed atomic action: for
%testing videos, the diversity of poses decreases 30\% compared to the previous
%model (QR), and 21\% compared to the new model using sparse regularizer but
%without considering the pose diversity penalty. All three models have similar
%accuracy on test videos, but the proposed sparse model produces each video to be
%represented by a small number of more representative learned poses.
%}


%\begin{figure*}[t]
%\begin{center}
%\includegraphics[width=0.95\linewidth]{./Influence_WH_modelGS_H.pdf} \\ (a) \\
%\includegraphics[width=0.95\linewidth]{./Influence_WH_model_H.pdf} \\ (b) \\
%\end{center}
%\caption{Influence of poses in activity \emph{Walk while calling with hands}. (a) using a sparse regularizer, (b) using a quadratic regularizer. The induced sparsity in the coefficients of action classifiers produces highly specialized poses. In this case, few poses are necessary to describe the arms (waving hand action), and more poses are needed to represent the walking action. Observing (a) we can speculate that most actors execute the \emph{waving hand} action using the right arm.}
%\label{fig:poses_decay_WH}
%%\vspace{-0.6cm}
%\end{figure*}
%
%\begin{figure*}[t]
%\begin{center}
%\includegraphics[width=0.95\linewidth]{./Influence_C6_modelGS_H.pdf} \\ (a) \\
%\includegraphics[width=0.95\linewidth]{./Influence_C6_model_H.pdf} \\ (b) \\
%\end{center}
%\caption{Influence of poses in activity \emph{Composed Activity 6}. (a) using a sparse regularizer, (b) using a quadratic regularizer. Comparing to Fig. \ref{fig:poses_decay_WH}, we can see that more poses influence this activity, which is expected since this activity is more complex than \emph{Walk while calling with hands}.}
%\label{fig:poses_decay_C6}
%%\vspace{-0.6cm}
%\end{figure*}


==> figures.tex <==


\begin{figure*}[ht]
\centering
 Motion poselet \#4 - most probable action: talking on cellphone\\
 \includegraphics[trim={0 0cm 0 0.5cm},clip,width=1.0\textwidth]{images/poselets1}

 Motion poselet \#7 - most probable action: erasing on board\\
 \includegraphics[trim={0 0cm 0 0.5cm},clip,width=1.0\textwidth]{images/poselets2}

 Motion poselet \#19 - most probable action: waving hand\\
 \includegraphics[trim={0 0cm 0 0.5cm},clip,width=1.0\textwidth]{images/poselets3}

 Motion poselet \#16 - most probable action: tennis swing\\
 \includegraphics[trim={0 0cm 0 0.5cm},clip,width=1.0\textwidth]{images/poselets4}

 Motion poselet \#34 - most probable action: golf swing\\
 \includegraphics[trim={0 0cm 0 0.5cm},clip,width=1.0\textwidth]{images/poselets5}

 Motion poselet \#160 - most probable action: bend\\
 \includegraphics[trim={0 0cm 0 0.5cm},clip,width=1.0\textwidth]{images/poselets6}

 \caption{set of poselets}
\end{figure*}


==> hierarchicalModel.tex <==
%\begin{comment}
%\subsection{Latent spatial actions for hierarchical action detection}
% %
%[CVPR2014 MODEL SUMMARY] In order to achieve or objectives, we build our model on top of the hierarchical model presented in \cite{Lillo2014}.
%The authors model an activity using three hierarchical levels: poses, atomic actions, and activities, using features extracted from 3D skeleton joints, splitting the human body into $R=4$ fixed spatial regions, corresponding to overlapping joints for arms and legs. It's a good sttr since the model considers energy potentials for poses as linear classifiers applied to frame features, selecting the pose classifier via a latent pose label $z_t \in \{1,\dots,K\}$. The pose modeling resembles Poselets [REF], In the mid-level of atomic actions, the model use as descriptor the BoW (histogram) representation of labels $Z$ for frames belonging to each action, in order to learn $A$ atomic action linear classifiers. The action label of a frame is denoted as $v_t \in \{1,\dots,A\}$. Finally, in the higher level of activities, the model use the BoW representation of actions labels $V$ of the video, to learn a multiclass linear classifier. Adding all energy terms, using $R=1$ for simplicity, and including temporal transition terms, the energy equation for video $D$ in \cite{Lillo2014} is 
%%
%\begin{eqnarray}
%\label{eq:energy2014}
%\begin{split}
%E(D) =  {\alpha_y}^\top h(V) + \sum_{a=1}^A {\beta_a}^\top h_a(Z) + \sum_{t=1}^T {w_{z_t}}^\top x_t  \\+ {\gamma}^\top h(V^{-1},V) + {\eta}^\top h(Z^{-1},Z)
%\end{split}
%\end{eqnarray}
%%
%where $h(V)$ is the histogram of atomic action labels, $h_a(Z)$ the histogram of pose labels at those frames labeled with action $a$, and $h(V^{-1},V)$ and $h(Z^{-1},Z)$ represents histograms for action and pose transitions respectively. The main idea is that the energy score for the video using the correct activity must be higher than every other activity. As during inference the labels $Z$ and $V$ are unknown, they must be inferred along with the activity label. Thus, an interesting property of this model is the per-frame nature of the energy function. The authors in \cite{Lillo2014} test their model in their own Composable Activities dataset, which include rich action labels annotated independently for four human regions (arms and legs). To date, this is the only action dataset with this level of spatial annotations. Our work take this model as an starting point to include flexibility... [CONTINUE]
%\end{comment}

\subsection{Hierarchical activity model}

Suppose we have a video $D$ with $T$ frames, each frame described by a feature vector $x_t$. Assume we have available $K$ classifiers$\{w_k\}_{k=1}^K$ over the frame descriptors, such that each frame descriptor can be associated to a single classifier. If we choose the maximum response for every frame, encoded as $z_t = \argmax_k\{w_k^\top x_t\}$,  we can build a BoW representation to feed linear action classifiers $\beta$, computing the histogram $h(Z)$ of $Z = \{z_1,z_2,\dots,z_T\}$ and using these histograms as a feature vector for the complete video to recognize single actions. Imagine now that we would like to use the scores of the maximum responses, $w_{z_t}^\top x_t$ as a potential to help discriminating between videos that present reliable poses from videos that does not. We can build a joint energy function, combining the action classifier score and the aggregated frame classifier scores, as
\begin{equation}
\label{eq:2-levels}
\begin{split}
E(D) &= \beta_{a}^\top h(Z) + \sum_{t=1}^T w_{z_t}^\top x_t \\ & = \sum_{t=1}^T\sum_{k=1}^K\left(\beta_{a,k} + w_k^\top x_t \right)\delta(z_t=k)
\end{split}
\end{equation}
What is interesting of Eq. (\ref{eq:2-levels}) is that it every term in the sum is tied for the value of $z_t$, creating a model such that all its components depends of the labeling $Z$. We can expand the previous model to more levels using the same philosophy. In fact, for a new level, we could create a new indicator $v_t$ for every frame that indicates the election of which classifier $\beta$ will be used (the same as $z_t$ indicates which classifier of $w$). If we name $w$ as \emph{pose classifiers}, and $\beta$ as \emph{action classifiers}, we can create a hierarchical model where multiple poses and actions can be present in a single video. Supposing we have $A$ actions; the energy for a three-level hierarchy could be, for an \emph{activity} $l$,
\begin{equation}
E(D) =\alpha_l^\top h(V) + \sum_{a=1}^A \beta_{a}^\top h^a(Z,V) + \sum_{t=1}^T w_{z_t}^\top x_t 
\end{equation}
where $h^a(Z,V)$ refers to the BoW representation of $Z$ for those frames labeled as action $v_t = a$.

[NEW MODEL]
%We propose three improvements to the model to make it more practical and flexible: firstly, to relax the need of action annotations for each human region, we propose to use latent variables representing the assignment of actions to human body regions; secondly, to overcome the multimodal representations of actions, we model each action as a group of linear classifiers instead of using a single classifier per action; and last, to handle the noisy or non-informative poses (NI), we propose a \emph{garbage collector} approach where the model itself identifies a threshold for the scores of pose classifiers of every human region. We describe each contribution in the following paragraphs.

Recent work in action recognition \cite{Cheron2015,Tao2015, Wang2011,Jhuang2013} shows a resurgence of describing human actions as a collection of dynamic spatial parts that resembles Poselets. In line with these research, we split the human body into $R$ semantic regions. As modeling actions using the whole body is hard, separating the body into groups of limbs helps in recognition of actions, specially for complex datasets \cite{Tao2015}. Our wiew is that while poses are in general well defined in most research, little effort has been made to mine actions from videos, in terms of detecting the temporal spanning (action detection) and action localization. In addition to the fact that most action datasets are only single actions, there is a lack of research in the general setup where actions are combined in the same video. Nevertheless, a few works have noticed that humans usually performs complex action in real life \cite{Wei2013, Lillo2014}, providing their own datasets based in RGB-D cameras. In our work, we aim to group both worlds of single and composed actions in a single hierarchical model of three semantic levels, and using human body regions to improve the representativeness. 

During training, we assume there is temporal annotations of actions. As we want our model to perform action localization, we model the action assignments $V_r$ in each region as latent variables during training, allowing the model to infer which human part execute the action without needing this kind of annotations in the training set, including a model for the initialization of action labels. In this way, we advance from a simple detection problem to infer also \emph{how} the subject executes the action, important in surveillance applications, health monitoring, between others. We also expand the modeling of recurrent patterns of poses to construct a general model for shared actions, aiming to handle multimodal information, which is produced by actions with the same label but with different execution patterns, or by changes in representation of actions such as varying camera view. We handle this problem by augmenting the number of action classifiers, where each original action acts as a parent node of several non-overlapping child actions. Finally, as we are using local information for poses, some frames could be noisy or representing an uncommon pose, not useful to build the pose models. We attack this issue by adding a garbage collector for poses, where only the most-informative poses are used by pose classifiers during learning. We describe these contributions in the following paragraphs.

\paragraph{[EDIT] Latent assignments of actions to human regions}

Knowing the parts of the body involved in the actions is highly appealing. Suppose we have $M$ videos, each video annotated with $Q_m$ action intervals. Each action interval can be associated with any number of regions, from $1$ to all $R$ regions. For example,  a \emph{waving hand} action could be associated only with \emph{right\_arm}, while the action \emph{jogging} could be associated with the whole body. We want to learn the associations of actions and human parts for training videos, and we build these associations using latent variables. The main problem to solve is to how to get a proper initialization for actions, since there is a very high chance to get sticked in a local minimum far away of the optimum, producing bad results.

Our first contribution is a method to get a proper initialization of fine-grained spatial action labels, knowing only the time span of the actions. Using the known action intervals,  we formulate the problem of action to region assignment as an optimization problem, constrained using structural information: the actions intervals must not overlap in the same region, and all the action intervals must be present at least in one region. We formulate this labeling problem as a binary Integer Linear Programming (ILP) problem. We define as $v_{r,q}^m=1$ when the action interval $q \in \{1,\dots,Q_m\}$ appears in region $r$ in the video $m$, and $v_{r,q}^m=0$ otherwise. We assume we have pose labels $z_{t,r}$ in each frame, independent for each region, learned via clustering the poses for all frames in all videos. For an action interval $q$, we use as descriptor the histogram of pose labels for each region in the action interval, defined for the video $m$ as $h_{r,q}^m$ . We can solve the problem of finding the correspondence between action intervals and regions in a formulation similar to $k$-means, using the structure of the problem as constraints in the labels, and using $\chi^2$ distance between the action interval descriptors and the cluster centers: 
\begin{equation}
\begin{split}
P1) \quad \min_{v,\mu} &\sum_{m=1}^M  \sum_{r=1}^R \sum_{q=1}^{Q_m}  v_{r,q}^m d( h_{r,q}^m - \mu_{a_q}^r) -\frac{1}{\lambda} v_{r,q}^m\\ 
 \text{s. to} 
\quad 
& \sum_{r=1}^R v_{r,q}^m \ge 1\text{, }\forall q\text{, }\forall m \\ 
%& \sum_{q=1}^{Q_m} v_{r,q}^m \le t_m \\ 
& v_{r,q_1}^m + v_{r,q_2}^m \le 1 \text{ if } q_1\cap q_2 \neq \emptyset \text{, }\forall r\text{, }\forall m\\  
& v_{r,q}^m \in \{0,1\}\text{, }\forall q\text{, }\forall{r}\text{, }\forall m
\end{split}
\end{equation}
with
\begin{equation}
d( h_{r,q}^m - \mu_{a_q}^r) = \sum_{k=1}^K (h_{r,q}^m[k] - \mu_{a_q}^r[k])^2/(h_{r,q}^m[k] +\mu_{a_q}^r[k]).
\end{equation}

$\mu_{a_q}^r$ are computed as the mean of the descriptors with the same action label within the same region. We solve $P1$ iteratively as $k$-means,  finding the cluster centers for each region $r$, $\mu_{a}^r$ using the labels $v_{r,q}^m$, and then finding the best labeling given the cluster centers, solving an ILP problem. Note that the first term of the objective function is similar to a $k$-means model, while the second term resembles the objective function of \emph{self-paced} learning as in \cite{Kumar2010}, fostering to balance between assigning a single region to every action, towards assigning all possible regions to the action intervals when possible.  

[IL: INCLUDE  FIGURE TO SHOW P1 GRAPHICALLY]

We describe the further changes in the hierarchical model of \cite{Lillo2014} in the learning and inference sections.
  \paragraph{[EDIT] Representing semantic actions with multiple atomic sequences}.


As the poses and atomic actions in \cite{Lillo2014} model are shared, a single classifier is generally not enough to model multimodal representations, that occur usually in  complex videos. We modify the original hierarchical model of \cite{Lillo2014} to include multiple linear classifiers per action. We create two new concepts: \textbf{semantic actions}, that refer to actions \emph{names} that compose an activity; and \textbf{atomic sequences}, that refers to the sequence of poses that conform an action. Several atomic sequences can be associated to a single semantic action, creating disjoint sets of atomic sequences, each set associated to a single semantic action.  The main idea is that the action annotations in the datasets are associated to semantic actions, whereas for each semantic action we learn several atomic sequence classifiers. With this formulation, we can handle the multimodal nature of semantic actions, covering the changes in motion, poses , or even changes in meaning of the action according to the context (e.g. the semantic action ``open'' can be associated to opening a can, opening a door, etc.). 

Inspired by \cite{Raptis2012}, we first use the \emph{Cattell's Scree test} for finding a suitable number of atomic sequence for every semantic action. Using the semantic action labels, we compute a descriptor for every interval using normalized histograms of pose labels. Then, for a particular semantic action $u$, we compute the the eigenvalues $\lambda_u$ of the affinity matrix of the semantic action descriptors, using $\chi^2$ distance. For each semantic action $u \in \{1,\dots,U\}$ we find the number of atomic sequences $G_u$ as $G_u = \argmin_i \lambda_{i+1}^2 / (\sum_{j=1}^i \lambda_j) + c\cdot i$, with $c=2\cdot 10^{-3}$. Finally, we cluster the descriptors corresponding to each semantic action using k-means, using a different number of clusters for each semantic action $u$ according to $G_u$. This approach generates non-overlapping atomic sequences, each associated to a single semantic action.

To transfer the new labels to the model, we define $u(v)$ as the function that given the atomic sequence label $v$, returns the corresponding semantic action label $u$. The energy for the activity level is then
\begin{equation}
E_{\text{activity}} =  \sum_{u=1}^U\sum_{t=1}^T \alpha_{y,u}\delta(u(v_t)=u)
\end{equation}  

For the action and pose labels the model remains unchanged. Using the new atomic sequences allows a richer representation for actions, while in he activity level, several atomic sequences will map to a single semantic action. This behavior resembles a max-pooling operation, where we will choose at inference the atomic sequences that best describe the performed actions in the video, keeping the semantics of the original labels. 

\paragraph{Towards a better representation of poses: adding a garbage collector}

The model in \cite{Lillo2014} uses all poses to feed action classifiers. Out intuition is that only a subset of poses in each video are really discriminative or informative for the actions performed, while there is plenty of poses that corresponds to noisy or non-informative ones. [EXPAND] Our intuition is that low-scored frames in terms of poses (i.e. a low value of $w_{z_t}^\top x_t$ in Eq. (\ref{eq:energy2014})) make the same contribution as high-scored poses in higher levels of the model, while degrading the pose classifiers at the same time since low-scored poses are likely to be related to non-informative frames. We propose to include a new pose, to explicitly handling those low-scored frames, keeping them apart for the pose classifiers $w$, but still adding a fixed score to the energy function to avoid normalization issues and to help in the specialization of pose classifiers. We call this change in the model a \emph{garbage collector} since it handles all low-scores frames and group them having a fixed energy score $\theta$. In practice, we use a special pose entry $K+1$ to identify the non-informative poses. The equation representing the energy for pose level is
%
\begin{equation} \label{Eq_poseEnergy}
E_{\text{poses}}  = \sum_{t=1}^T \left[  {w_{z_t}}^\top x_{t}\delta(z_{t} \le  K) + \theta 
\delta(z_{t}=K+1)\right] 
\end{equation}
where $\delta(\ell) = 1$ if $\ell$ is true and $\delta(\ell) = 0$ if
$\ell$ is false. The action level also change its energy:
\begin{equation}
\begin{split}
 \label{Eq_actionEnergy}
E_{\text{actions}} =  \sum_{t=1}^T \sum_{a=1}^A \sum_{k=1}^{K+1}  \beta_{a,k} \delta(z_t = k) \delta(v_t = a).
\end{split}
\end{equation}

\begin{comment}
Integrating all contribution detailed in previous sections, the model is written as:
Energy function:
\begin{equation}
E = E_{\text{activity}} + E_{\text{action}} + E_{\text{pose}}
  + E_{\text{action transition}} + E_{\text{pose transition}}.
\end{equation}

\begin{equation}
E_{\text{poses}}  = \sum_{t=1}^T \left[  {w_{z_t}}^\top x_{t}\delta(z_{t} \le  K) + \theta 
\delta(z_{t}=K+1)\right] 
\end{equation}

\begin{equation}
E_{\text{actions}} =  \sum_{t=1}^T \sum_{a=1}^A \sum_{k=1}^{K+1}  \beta_{a,k} \delta(z_t = k) \delta(v_t = a).
\end{equation}

\begin{equation}
h_g^{r}(U) = \sum_{t} \delta_{u_{t,r}}^g
\end{equation}

So the energy in the activity level is
\begin{equation}
E_{\text{activity}} = \sum_{r} {\alpha^r_{y}}^\top h^{r}(U) = \sum_{r,g,t}  \alpha^r_{y,g} \delta_{u_{t,r}}^g
\end{equation}

\begin{equation}
E_{\text{action transition}} = \sum_{r,a,a'}  \gamma^r_{a',a} \sum_{t} \delta_{v_{t-1,r}}^{a'}\delta_{v_{t,r}}^a 
\end{equation}

\begin{equation}
E_{\text{pose transition}} =\sum_{r,k,k'}  \eta^r_{k',k}\sum_{t}\delta_{z_{t-1,r}}^{k'}\delta_{z_{t,r}}^{k}
\end{equation}
\end{comment}




==> introduction_IL.tex <==
[IL addings]
 
Many benchmarks in action recognition are constructed using short videos of single human actions. As \cite{Lillo2014} and \cite{Wei2013} noticed, in a more realistic setup the  subjects are able to execute several actions at the same time, like waving a hand while calling by cellphone. This setups are known as \emph{complex}, \emph{composed}, or \emph{concurrent} actions according to the context. Using this kind of action configuration makes the inference difficult since we are dealing with a spatio/temporal multilabel setup: in a single video, multiple actions can appear, and they can be temporally or spatially composed. Models like \cite{Lillo2014}, \cite{Wei2013} addresses composed actions, both providing a new dataset using RBG-B sensors. On the other hand, a benchmark that issue single actions per video can benefit of a more complex model, identifying  temporal or spatial segments where the action actually occurs. While several models exists for single actions, only few models have been developed to tackle composed or concurrent actions.

In \cite{Lillo2014}, the authors provide the \emph{Composable Activities} dataset, where the atomic actions were fully annotated temporally and spatially: each human region (4 regions) have a different set of temporal annotations of actions, which make this dataset unique. However, this fact also makes the model created in top of this dataset not very useful for a more general setup, where only the temporal spanning of concurrent actions are annotated. In fact, databases of simple actions should be augmented in annotations,  which make the model not general for most action datasets. We improve the model in \cite{Lillo2014} by treating the spatial assignments of actions as latent variables. 

==> videoRepresentation.tex <==
\subsection{Video Representation} \label{subsec:videorepresentation}

[EXPLAIN BETTER, ADD FIGURE]
Our model is based on skeleton information encoded in joint annotations.  We use the same geometric descriptor as in \cite{Lillo2014}, using angles between segments connecting two joints, and angles between these segments and a plane formed by three joints. In addition to geometry, other authors \cite{Zanfir2013,Tao2015,Wang2014} have noticed that including local motion information is beneficial to the categorization of videos. Moreover, in \cite{zhu2013fusing} the authors create a fused descriptor using spatio-temporal descriptors and joint descriptors, showing that they combined perform better than separated. With this is mind, we augment the original geometric descriptor with motion information: when there is only skeleton jonints data, we use the displacement of vectors (velocity) as a motion descriptor. If RGB video is available, we use the HOF descriptor extracted from the trajectory of the joint in a small temporal window.

For the geometric descriptor, we use 6 segments per human action (see Fig. XXXX). The descriptor is composed by the angles between the segments (15 angles), and the angles between a plane formed by three segments and the non-coplanar segments (3 angles). For motion descriptor, we use either the 3D velocity of every joint in each region as a concatenated vector (18 dimensions), or the concatenated HOF descriptor of the joint trajectories, transformed to a low-dimensional space using PCA (20 dimensions).

